Verification of Neural Control Barrier Functions with Symbolic Derivative Bounds Propagation

Control barrier functions (CBFs) are important in safety-critical systems and robot control applications. Neural networks have been used to parameterize and synthesize CBFs with bounded control input for complex systems. However, it is still challenging to verify pre-trained neural networks CBFs (neural CBFs) in an efficient symbolic manner. To this end, we propose a new efficient verification framework for ReLU-based neural CBFs through symbolic derivative bound propagation by combining the linearly bounded nonlinear dynamic system and the gradient bounds of neural CBFs. Specifically, with Heaviside step function form for derivatives of activation functions, we show that the symbolic bounds can be propagated through the inner product of neural CBF Jacobian and nonlinear system dynamics. Through extensive experiments on different robot dynamics, our results outperform the interval arithmetic based baselines in verified rate and verification time along the CBF boundary, validating the effectiveness and efficiency of the proposed method with different model complexity. The code can be found at https://github.com/intelligent-control-lab/ verify-neural-CBF.

==> old_method.tex <==
\section{Method}
\subsection{Linear Bounds of Non-linear Affine System}
We first study the linear bounds of the general control-affine system 
with hyper-rectangle bounded input  $\v u\in[\underline{\v u}, \overline{\v u}]:=\{\v u\in\mathbb{R}^m\mid \underline{\v u}\leq \v u\leq \overline{\v u}\}$ and hyper-rectangle bounded state  $\v x\in[\underline{\v x}, \overline{\v x}]:=\{\v x\in\mathbb{R}^n\mid \underline{\v x}\leq \v x\leq \overline{\v x}\}$ as $$\dot{\v x} = h(\v x, \v u) = f(\v x) + g(\v x) \v u, \v u\in[\underline{\v u}, \overline{\v u}], \v x\in[\underline{\v x}, \overline{\v x}]$$
where $h(\v x, \v u)$ is analytical and its second-order derivative exists. We have the following lemma to find feasible  linear lower and upper bounds of $f(\v x)$ and $g(\v x)$  as $\underline{f}(\v x) \leq f(\v x) \leq \overline{f}(\v x)$ and $\underline{g}(\v x) \leq g(\v x) \leq \overline{g}(\v x)$.
\begin{lemma}\label{lemma:bound_system}
     For the general control-affine system $\dot{\v x} = h(\v x, \v u) = f(\v x) + g(\v x) \v u$ with bounded state and control input $\underline{\v x} \leq \v x\leq \overline{\v x}, \underline{\v u} \leq \v u\leq \overline{\v u}$, suppose the Jacobian can be bounded as $\underline{\v{\nabla}}_{\v x} \leq \nabla_{\v x} h(\v x,\v u) \leq \overline{\v{\nabla}}_{\v x}  $  and $\underline{\v{\nabla}}_{\v u}  \leq \nabla_{\v u} h(\v x,\v u) \leq \overline{\v{\nabla}}_{\v u}  $, and the $\ell_2$ operator norm of Hessian matrix of $i$-th entry of $h(\v x,\v u)$ is bounded as $\max_{\underline{\v u} \leq \v u\leq \overline{\v u}}\|\nabla_{\v x}^2 h^{(i)}(\v x,\v u)\|_2\leq M^{(i)}$, then given $ \v u_0\in[\underline{\v u}, \overline{\v u}], \v x_0\in[\underline{\v x}, \overline{\v x}]$ the following linear bounds can be found as
     \begin{align}
     \label{eq:linear_dyn}
          \underline{\v W}_{f} \v x+ \underline{\v b}_{f}\leq f(\v x)\leq \overline{\v W}_{f} \v x+ \overline{\v b}_{f},\underline{\v W}_{g} \v x+ \underline{\v b}_{g}\leq g(\v x)\leq \overline{\v W}_{g} \v x+ \overline{\v b}_{g}
     \end{align}
     where $\underline{\v W}_{f} = {\nabla}_{\v x}^\top h(\v x_0, \v u_0) , \overline{\v W}_{f} =
     {\nabla}_{\v x}^\top h(\v x_0, \v u_0) ,\underline{\v W}_{g} = \overline{\v W}_{g} =
     \mathbf{0}, \underline{\v b}_{g} = \underline{\v{\nabla}}_{\v u}, \overline{\v b}_{g} = \overline{\v{\nabla}}_{\v u}$ and
     $
     \underline{\v b}_{f}^{(i)} = h^{(i)}(\v x_0, \v u_0) - {\nabla}_{\v x}^\top h^{(i)}(\v x_0, \v u_0) \v x_0 - \frac{1}{2}\|\overline{\v x} - \underline{\v x}\|_2^2 M^{(i)} -\underline{\v{\nabla}}_{\v u}^{\top(i)}  [\v u_{0}]_- -\overline{\v{\nabla}}_{\v u}^{\top(i)}  [\v u_{0}]_+,~~ \overline{\v b}_{f}^{(i)} = h^{(i)}(\v x_0, \v u_0) - {\nabla}_{\v x}^\top h^{(i)}(\v x_0, \v u_0) \v x_0 + \frac{1}{2}\|\overline{\v x} - \underline{\v x}\|_2^2 M^{(i)} -\underline{\v{\nabla}}_{\v u}^{\top(i)}  [\v u_{0}]_+ -\overline{\v{\nabla}}_{\v u}^{\top(i)}  [\v u_{0}]_-
     $  for each $i$-th entry.
     
         Specifically, if the control-affine system is linear and time-invariant, \ie, $f(\v x) = \v A \v x$ and $g(\v x) = \v B$ with constant $\v A, \v B$, where the lower and upper bounds will trivially be $\underline{\v W}_{f} = \overline{\v W}_{f} =\v A, \underline{\v W}_{g} = \overline{\v W}_{g} =\v 0,\underline{\v b}_{f} = \overline{\v b}_{f}=\v 0,  \underline{\v b}_{g} = \overline{\v b}_{g}=\v B.$
\end{lemma}
% \begin{remark}

    %     \begin{align}
    %     &\max_{\v x\in \Delta\mathcal{X}_k} \min_{\v u\in[\underline{\v u}, \overline{\v u}]} \nabla_{\v x} \phi^\top(\v x)(f(\v x)+g(\v x)\v u) \leq [\overline{\v f}_k^\top]_-[\underline\nabla_k(\v x)]_++[\underline{\v f}_k^\top]_-[\underline\nabla_k(\v x)]_- + [\overline{\v f}_k^\top]_+[\overline\nabla_k(\v x)]_+ +\notag\\ &[\underline{\v f}_k^\top]_+[\overline\nabla_k(\v x)]_- + [\underline \nabla_k^\top(\v x)]_-[\underline{\v g}_k]_-\underline{\v u} + [\overline \nabla_k^\top(\v x)]_+[\overline{\v g}_k]_+\underline{\v u} + [\underline\nabla_k^\top(\v x)]_+[\overline{\v g}_k]_-\overline{\v u} + [\overline \nabla_k^\top(\v x)]_-[\underline{\v g}_k]_+\overline{\v u}
    % \end{align}
% \end{remark}

\subsection{Verification of Neural CBF with Linearly Bounded Dynamics}
Given the hyper-rectangle bounded input  $\v u\in[\underline{\v u}, \overline{\v u}]:=\{\v u\in\mathbb{R}^m\mid \underline{\v u}\leq \v u\leq \overline{\v u}\}$, based on interval arithmetic \cite{liu2021algorithms}, we have the following lemma to have the equivalent expression of the inner minimization in Eq. \eqref{eq:goal}.
\begin{lemma}
    When $\v u$ is within a hyper-rectangle $\mathcal{U}=[\underline{\v u}, \overline{\v u}]=\{\v u\in\mathbb{R}^m\mid \underline{\v u}\leq \v u\leq \overline{\v u}\}$, given $\v x\in\mathcal{X}$, the minima of $\dot \phi(\v x)= L_f\phi(\v x) + L_g\phi(\v x) {\v u}$ over $\v u$ can be found explicitly as,
    \begin{align}
        \min_{\v u\in\mathcal{U}}  L_f\phi(\v x) + L_g\phi(\v x) {\v u}= L_f\phi(\v x) + [L_g\phi(\v x)]_+ \underline{\v u} +[L_g\phi(\v x)]_- \overline{\v u}
    \end{align}
    where $[\cdot]_+= \max\{0, \cdot\}, [\cdot]_-= \min\{0, \cdot\}$.
\end{lemma}
% \begin{proposition}
%     Given $\underline{u}\leq u\leq \overline{u}\in \mathbb{R}^m$, the following bounds hold for any linear transformation $Wu+b$,
%     \begin{align}
%         [W]_+ \underline u+[W]_- \overline u + b\leq Wu+b \leq [W]_- \underline u+[W]_+ \overline u + f(\v x)
%     \end{align}
%     where $[\cdot]_+= \max\{0, \cdot\}$ and $[\cdot]_-= \min\{0, \cdot\}$.
% \end{proposition}
Therefore, the verification goal of Eq. \eqref{eq:goal} can be equivalently written as,
\begin{align}
\label{eq:goal_x}
    % &\max_{\v x\in \partial \mathcal{X}_\phi(\v x)} \min_{\v u\in\mathcal{U}} \nabla_{\v x} \phi^\top(\v x)(f(\v x)+g(\v x)\v u)\notag\\=&
    \max_{\v x\in \partial \mathcal{X}_\phi(\v x)} \nabla_{\v x} \phi^\top f(\v x) + [\nabla_{\v x} \phi^\top g(\v x)]_+ \underline{\v u} +[\nabla_{\v x} \phi^\top g(\v x)]_- \overline{\v u}  \leq 0
\end{align}
Suppose all the roots of $\phi(\v x)=0$ can be over-approximated by the union set of $K$ hyper-rectangle $ \cup_{k=1}^K \Delta\mathcal{X}^{(k)}$, i.e. 
$$\partial \mathcal{X}_\phi\subset  \cup_{k=1}^K \Delta\mathcal{X}^{(k)}, \text{ where } \Delta\mathcal{X}^{(k)}=\{\v x\mid \underline x^{(k)} \leq \v x \leq \overline x^{(k)} \}.$$

Within each hyper-rectangle bounded state set $\Delta \mathcal{X}$, based on Lemma \ref{lemma:bound_system}, the control-affine system  can be bounded by linear lower and upper bounds as $f(\v x) \in [\underline{f}(\v x), \overline{f}(\v x)], g(\v x)\in[\underline{g}(\v x), \overline{g}(\v x)]$.
Then we have the following theorem to upper-bound  $ L_f\phi(\v x) + L_g\phi(\v x) {\v u}$ with input set $[\underline{\v u}, \overline{\v u}]$
\begin{theorem}
\label{thm:symbolic_bound_dyn}
    For any hyper-rectangle bounded state $\v x\in \Delta \mathcal{X}$ and any hyper-rectangle bounded input $\v u\in  \mathcal{U}=[\underline{\v u}, \overline{\v u}]$,  the dynamic system is bounded as $ \underline{f}(\v x)\leq f(\v x)\leq \overline{f}(\v x), \underline{g}(\v x)\leq g(\v x)\leq \overline{g}(\v x)$,  then it holds for $\dot\phi=L_f\phi(\v x) + L_g\phi(\v x) {\v u}$ that
    % we have the linear upper bound for Eq. \eqref{eq:goal} and \eqref{eq:goal_x} as
    \begin{align*}
        \max_{\v x\in \Delta\mathcal{X}} \min_{\v u\in\mathcal{U}}  \dot\phi \leq \overline{L}_f\phi(\v x) + [\overline{L}_g\phi(\v x) ]_+[\underline{\v u}]_+ + [\underline{L}_g\phi(\v x) ]_+[\underline{\v u}]_-  + [\overline{L}_g\phi(\v x) ]_-[\overline{\v u}]_+ + [\underline{L}_g\phi(\v x) ]_-[\overline{\v u}]_-
    \end{align*}
    where $[\cdot]_+= \max\{0, \cdot\}$,  $[\cdot]_-= \min\{0, \cdot\}$ and the lower and upper bound of Lie derivatives are 
    \begin{align*}
        &\underline{L}_f\phi(\v x) 
 = [\nabla_{\v x} \phi^\top ]_+ \underline{f}(\v x) + [\nabla_{\v x} \phi^\top ]_-\overline{f}(\v x),~ \overline{L}_f\phi(\v x) 
 = [\nabla_{\v x} \phi^\top ]_+ \overline{f}(\v x) + [\nabla_{\v x} \phi^\top ]_-\underline{f}(\v x) \\
 & \underline{L}_g\phi(\v x) 
 = [\nabla_{\v x} \phi^\top ]_+ \underline{g}(\v x) + [\nabla_{\v x} \phi^\top ]_-\overline{g}(\v x),~ \overline{L}_g\phi(\v x) 
 = [\nabla_{\v x} \phi^\top ]_+ \overline{g}(\v x) + [\nabla_{\v x} \phi^\top ]_-\underline{g}(\v x)
    \end{align*}
\end{theorem}
% Then the  upper-bound  of  Eq. \eqref{eq:goal_x},


\subsection{Efficient Bound Propagation for Lie Derivative}
% First show how to make activation as box for gradient, then show the IBP case, add a remakr to show that ours can be degraded to existing one if f and g are boxes
Now we consider the neural network parameterization of CBF $\phi: \mathbb{R}^n\rightarrow \mathbb{R}$. Generally, the neural CBF consists of $L$ feedforward layers $h_i:\mathbb{R}^{n_{i-1}}\rightarrow\mathbb{R}^{n_i}, i=1,2,\dots,L$, associated with $L-1$  element-wise non-linear activation functions (ReLU, sigmoid, tanh, etc) $\sigma_i: \mathbb{R}^{n_i}\rightarrow \mathbb{R}^{n_i},i =1,2,\dots, L-1$ after each linear feedforward layer. Therefore, the neural CBF is formulated as the compositional function below
\begin{align}
    \phi(\v x)= h_L \circ \sigma_{L-1} \circ h_{L-1}\circ \sigma_{L-2} \circ h_{L-2}\cdots \circ \sigma_{1} \circ h_{1}(\v x)
\end{align}
where $h_i:\mathbb{R}^{n_{i-1}}\rightarrow\mathbb{R}^{n_i}, \sigma_i: \mathbb{R}^{n_i}\rightarrow \mathbb{R}^{n_i}$ and $n_0=n, n_L=1$. Furthermore, each feedforward layer $h_i$ is parameterized with weight $\v W_i\in\mathbb{R}^{n_i\times n_{i-1}}$ and bias $\v b_i\in\mathbb{R}^{n_i}$ as $\hat{\v z}_i = h_i(\v z_{i-1}) = \v W_{i}\v z_{i-1} + \v b_i$, where $\hat{\v z}_{i-1}\in \real^{n_i}$ is the pre-activation output of $h_i$ and  $\v z_{i-1}\in\real^{n_{i-1}}$ is the output of last activation layer $\v z_{i-1} = \sigma_{i-1}(\hat{\v z}_{i-1})$. Besides, it holds trivially for the initial and final intermediate vectors that $\hat{\v z}_L=\phi(\v x), \v z_0=\v x$.

For the gradients  of $\phi$ with respect to  intermediate vectors $\v z_{i-1}, \hat{\v z}_{i}, \forall i= 1,2,\dots,L$, based on chain rule, we have
\begin{align}
\label{eq:recursive}
    \nabla_{\v z_{i-1}}\phi = \nabla_{\v z_{i-1}}^\top h_i \nabla_{\hat{\v z}_i}\phi = \v W_i^\top \nabla_{\hat{\v z}_i}\phi, ~ \nabla_{\hat{\v z}_{i}}\phi = \frac{\partial \v z_i}{\partial \hat{\v z}_i}\odot \nabla_{\v z_{i}}\phi = \sigma'(\hat{\v z}_i)\odot \nabla_{\v z_{i}}\phi
\end{align}
where $\odot$ denotes element-wise Hadamard product for two inputs with the same size. Based on the initial condition $\nabla_{\hat{\v z}_L}\phi = \v I$, the recursive formula in Eq. \eqref{eq:recursive} will result in the gradient w.r.t the input $\nabla_{\v x}\phi = \nabla_{\v z_0}\phi$ in a back-propagation manner.

Although previous work has shown that the Jacobian  of neural networks $\nabla_{\v x} \phi$ can be linear bounded w.r.t the input $\v x$ as follows based on the linear bounds of ReLU activation 
\begin{align}
\label{eq:jacobian}
    \underline\nabla(\v x) = \underline{\v \Lambda} \v x + \underline{\v d} \leq \nabla_{\v x} \phi\leq\overline\nabla(\v x) =  \overline{\v \Lambda} \v x + \overline{\v d}
\end{align}
such general lower and upper linear bounds $\underline\nabla(\v x), \overline\nabla(\v x)$ make finding the lower and upper bounds of Lie derivatives in Thm. \ref{thm:symbolic_bound_dyn} intractable due to the quadratic programming with linear constraints. Besides, it is not clear how to extend the linear bound to other differential activation functions like sigmoid and tanh, which have been widely used in the literature on neural CBF. To this end, we propose the following theorem to further characterize the properties of Eq. \eqref{eq:jacobian} in a more general way.
\begin{theorem}
\label{thm:general_jacobian}
For any feedforward neural networks associated with any non-linear activation function $\sigma_i, i=1,2,\dots,L-1$, given $\ell_\infty$ bounded input $\v x$, if the derivative of each activation function $\sigma_i$ is bounded as  $\underline{\v \sigma}_i'\leq \sigma_i'(\hat{\v z}_i)\leq \overline{\v \sigma}_i'$, the linear bounds of gradient $\nabla_{\v x}\phi$  will be degraded as
\begin{align}
\label{eq:box_jacobian}
    \underline\nabla(\v x) = \underline{\v \Lambda} \v x + \underline{\v d} \leq \nabla_{\v x} \phi\leq\overline\nabla(\v x) =  \overline{\v \Lambda} \v x + \overline{\v d}, \text{ where } \underline{\v \Lambda}=\overline{\v \Lambda} = \v 0
\end{align}
Then given the linear bounds $\underline{f}(\v x)=\underline{\v W}_{f}^{(k)} \v x+ \underline{\v b}_{f}^{(k)}\leq f(\v x)\leq \overline{f}(\v x) =\overline{\v W}_{f}^{(k)} \v x+ \overline{\v b}_{f}^{(k)}$,
the lower and upper bound of Lie derivative $L_f\phi(\v x)$ will be 
\begin{align}
\label{eq:lie_grad}
&\underline{L}_f\phi(\v x) 
 = [\overline{\v d}^\top]_+ [\underline{f}(\v x)]_- + [\underline{\v d}^\top]_+[\underline{f}(\v x)]_++[\overline{\v d}^\top]_- [\overline{f}(\v x)]_- + [\underline{\v d}^\top]_-[\overline{f}(\v x)]_+\\& \overline{L}_f\phi(\v x) 
 = [\overline{\v d}^\top]_+ [\overline{f}(\v x)]_- + [\underline{\v d}^\top]_+[\overline{f}(\v x)]_-+[\overline{\v d}^\top]_- [\underline{f}(\v x)]_+ + [\underline{\v d}^\top]_-[\underline{f}(\v x)]_-,
\end{align}
where $[\cdot]_+= \max\{0, \cdot\}$,  $[\cdot]_-= \min\{0, \cdot\}$, then the upper bound of $\dot\phi = L_f\phi(\v x) + L_g\phi(\v x)\v u$ can be found in the same way as Thm. \ref{thm:symbolic_bound_dyn}.
\end{theorem}
\begin{remark}
    We remark that the constant bounded gradient of the activation function holds generally for ReLU \cite{shi2022efficiently}, sigmoid, tanh, etc. Moreover, if the dynamics $f(\v x), g(\v x)$ can be  bounded by constant, the symbolic  bounds of Eq. \eqref{eq:lie_grad} can be  degraded  to the vertices case \cite{wang2023simultaneous}, showing our bound is more general and tighter.
\end{remark}

% If the Jacobian of the neural CBF $\nabla_{\v x} \phi^\top $ can be  bounded as $\underline\nabla_k  \leq \nabla_{\v x} \phi(\v x)\leq\overline\nabla_k$, the symbolic upper bound of Eq. \eqref{eq:symbolic_bound} can be further relaxed to the vertices case [cite simult], showing our bound is more general and tighter. Furthermore 


==> relatedwork.tex <==
\section{Related Work}
recent Lyapunov \cite{yang2024lyapunov}, no barrier

==> training.tex <==


\subsection{Lagrange Duality for Model Training}
Now we model the neural CBF using the logits difference of a binary classification with input of state $\v x$ and labels  $y=\mathbbm{1}(\v x\in\mathcal{X}_S)$. Specifically, if the neural network $h_\theta: \mathcal{X}\rightarrow\mathbb{R}^2$ predicts the logits of the binary classification, neural CBF can be directly constructed as 
$$\phi_\theta(\v x) = [1 -1] h_\theta(\v x), \text{ where } p(y\mid \v x) = \text{softmax}(h_\theta(\v x))$$
Therefore, the time derivative of neural CBF $\dot\phi_\theta$ can also be parameterized by $h_\theta$ based on the following proposition.
\begin{proposition} Given any continuous functions $h_\theta: \mathbb{R}^n\rightarrow\mathbb{R}^2$  with input state dynamics $\dot{\v x} = f(\v x) + g(\v x) \v u, \v u\in\mathbb{R}^m$, if $\phi_\theta(\v x) = [1 -1] h_\theta(\v x)$, it holds that
\begin{align}
\label{eq:cbf_h}
    \dot\phi_\theta(\v x) = \nabla_{\v x} \phi_\theta^\top(\v x)(f(\v x)+g(\v x)\v u) = [1 -1] \nabla_{\v x}h_\theta^\top(\v x)(f(\v x) + g(\v x) \v u) =[1 -1] \dot h_\theta(\v x)
\end{align}
\end{proposition}


If $h_\theta$ is parameterized as feedforward neural networks with ReLU activation layers, based on , we have the linear lower bounds and upper bounds for the gradient $\nabla_{\v x} \phi_\theta(\v x)=[1 -1]^\top \nabla_{\v x} h_\theta(\v x)$ for $\v x\in\Delta\mathcal{X}_k$ as
\begin{align}
\label{eq:jacobian}
    \underline\nabla_k(\v x) = \underline{\v \Lambda}_k \v x + \underline{\v d}_k \leq \nabla_{\v x} \phi_\theta(\v x)=[1 -1]^\top \nabla_{\v x} h_\theta(\v x) \leq\bar\nabla_k(\v x) =  \bar{\v \Lambda}_k \v x + \bar{\v d}_k
\end{align}
